Approximate Logic Synthesis Using BLASYS

Approximate computing is an emerging paradigm where design accuracy can be traded for improvements in design metrics such as design area and power consumption. In this work, we overview our open-source tool, BLASYS, for synthesis of approximate circuits using Boolean Matrix Factorization (BMF). In our methodology the truth table of a given circuit is approximated using BMF to a controllable approximation degree, and the results of the factorization are used to synthesize the approximate circuit output. BLASYS scales up the computations to large circuits through the use of partition techniques, where an input circuit is partitioned into a number of interconnected subcircuits and then a design-space exploration technique identifies the best order for subcircuit approximations. BLASYS leads to a graceful trade-off between accuracy and full circuit complexity as measured by design area. Using an open-source design flow, we extensively evaluate our methodology on a number of benchmarks, where we demonstrate that the proposed methodology can achieve on average 48.14% in area savings, while introducing an average relative error of 5%.

==> prev_work.tex <==
%!TEX root =  bare_conf.tex

%There are two lines of research in approximate synthesis. The first line of research has devised custom approximate designs for typical arithmetic building blocks (e.g., adders, multipliers, dividers \cite{Hu,Kahng,drum,Rehman,Imani1}). The second line has targeted approximation of more generic circuits. For generic circuits, some techniques have been proposed to generate approximate circuits from gate-level (i.e., Boolean descriptions) \cite{LiL15,salsa,aslan14,sasimi,Miao13,Miao14}, higher-level descriptions, such as RTL or behavioral descriptions \cite{Nepal14}, or even direct C to approximate hardware synthesis \cite{Lee17}.  

Recent work on approximate circuit synthesis can be divided into two general categories: Boolean or gate-level approaches and high-level synthesis approaches.

For Boolean and gate-level synthesis, a number of approaches have been proposed \cite{salsa,aslan14,sasimi,Miao13,Vasicek2016}. In SALSA, a systematic approach for approximate circuit synthesis is proposed \cite{salsa}. The idea is to create a difference circuit that compares the QoR between the original circuit and the approximated circuit. The don't cares of the outputs of the approximate circuit -- which are internal nodes in the difference circuit -- with respect to outputs of the difference circuit can be used to simplify the approximate circuit using regular logic synthesis techniques. This approach has been extended in ASLAN~\cite{aslan14} to model error arising over multiple cycles. ASLAN also uses a circuit block exploration method that identifies the impact of approximating the combinational blocks and then uses a gradient-descent approach to find good approximations for the entire circuit. In SASIMI ~\cite{sasimi}, a technique is proposed to identify similar signals, such that their values agree over a large number of input test cases, and then substitute one for the other, simplifying the logic. A logic synthesis formulation proposed by Miao {\it et al.} uses a two-level logic synthesis approach that incorporates constraints on error deviation, and then a heuristic is used to solve the synthesis formulation \cite{Miao13}. Evolutionary techniques have been also explored~\cite{Vasicek2016}.

For high-level logic synthesis, ABACUS seeks to generate variants of an input high-level Verilog description file by applying a set of possible transformations, such as  bit width truncation, operand simplification and variable-to-constant substitution, to generate a set of mutant approximate circuit variants \cite{Nepal14}. A multi-objective design space exploration technique is used to identify the best set of approximate variants.  Recently, a new technique is proposed to raise the level of abstraction by synthesizing approximate circuit directly from C descriptions \cite{Lee17}. High-level synthesis in conjunction with approximations on the critical path can yield additional savings through voltage scaling \cite{TETC16,Lee17}.

%\vspace{2.5in}
